LM-Gaussian: Boost Sparse-view 3D Gaussian Splatting with Large Model Priors

We aim to address sparse-view reconstruction of a 3D scene by leveraging priors from large-scale vision models. While recent advancements such as 3D Gaussian Splatting (3DGS) have demonstrated remarkable successes in 3D reconstruction, these methods typically necessitate hundreds of input images that densely capture the underlying scene, making them time-consuming and impractical for real-world applications. However, sparse-view reconstruction is inherently ill-posed and under-constrained, often resulting in inferior and incomplete outcomes. This is due to issues such as failed initialization, overfitting on input images, and a lack of details. To mitigate these challenges, we introduce LM-Gaussian, a method capable of generating high-quality reconstructions from a limited number of images. Specifically, we propose a robust initialization module that leverages stereo priors to aid in the recovery of camera poses and the reliable point clouds. Additionally, a diffusion-based refinement is iteratively applied to incorporate image diffusion priors into the Gaussian optimization process to preserve intricate scene details. Finally, we utilize video diffusion priors to further enhance the rendered images for realistic visual effects. Overall, our approach significantly reduces the data acquisition requirements compared to previous 3DGS methods. We validate the effectiveness of our framework through experiments on various public datasets, demonstrating its potential for high-quality 360-degree scene reconstruction. Visual results are on our website.

==> main/8_references.tex <==
\section*{References}
\begin{thebibliography}{8}
\bibitem{Nerf}
{Mildenhall, B., Srinivasan, P.P., Tancik, M., Barron, J.T., Ramamoorthi, R., \& Ng, R. (2020). NeRF. Communications of the ACM, 65, 99 - 106.}
\bibitem{3DGS}
Kerbl, B., Kopanas, G., Leimkuehler, T., \& Drettakis, G. (2023). 3D Gaussian Splatting for Real-Time Radiance Field Rendering. ACM Transactions on Graphics (TOG), 42, 1 - 14.
\bibitem{LLFF}
Mildenhall, B. (2019). Local Light Field Fusion: Practical View Synthesis with Prescriptive Sampling Guidelines.
\bibitem{Metric3D}
Hu, M., Yin, W., Zhang, C., Cai, Z., Long, X., Chen, H., Wang, K., Yu, G., Shen, C., \& Shen, S. (2024). Metric3D v2: A Versatile Monocular Geometric Foundation Model for Zero-shot Metric Depth and Surface Normal Estimation.
\bibitem{Tanksandtemple}
Knapitsch, A., Park, J., Zhou, Q., \& Koltun, V. (2017). Tanks and temples. ACM Transactions on Graphics (TOG), 36, 1 - 13.
\bibitem{LPIPS}
Zhang, R., Isola, P., Efros, A.A., Shechtman, E., \& Wang, O. (2018). The Unreasonable Effectiveness of Deep Features as a Perceptual Metric. 2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition, 586-595.
\bibitem{SSIM}
Wang, Z., Bovik, A.C., Sheikh, H.R., \& Simoncelli, E.P. (2004). Image quality assessment: from error visibility to structural similarity. IEEE Transactions on Image Processing, 13, 600-612.
\bibitem{RaDe-GS}
{Zhang, Baowen et al. “RaDe-GS: Rasterizing Depth in Gaussian Splatting.” ArXiv abs/2406.01467 (2024): n. pag.}
\end{thebibliography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


